WEQA: Wearable hEalth Question Answering with Query-Adaptive Agentic Reasoning

Language models are remarkably capable at medical question answering, in some cases surpassing the accuracy of general physicians. However, answering questions about wearable health data remains challenging and understudied, as these ubiquitous sensors produce continuous, high-dimensional, and longitudinal data, which is non-trivial to align with text-centric distributions in LLM pretraining. The diversity of sensor modalities and user intents cannot be effectively handled by a fixed reasoning workflow or a single pretrained foundation model. To address these challenges, we propose WEQA, a query-adaptive agent framework that unifies LLM reasoning with specialized wearable analytical and modeling tools. An LLM controller is employed to synthesize execution plans and dynamically route each query to the appropriate combination of sensor analysis and pretrained models, and perform grounded response auditing with external knowledge. We also curate a benchmark spanning four open wearable datasets comprising analytic and predictive tasks in three different health domains. Experiments show that our framework is 24% more accurate than LLM and agentic baselines, and a blinded study with 12 medical experts and 8 users shows substantial gains in usefulness and clinical soundness.

==> tables/plan.tex <==
\begin{observationbox}
\small
\textbf{Example Execution Plan.} \\

Query: \textit{How many steps did I take in the hour of my maximum heart rate today?} \\
\textbf{Objective:} Find the total steps during the hour of maximum heart rate for the current day. \\
\textbf{Task type:} Data retrieval \\
\textbf{Required data:} Heart rate, step count \\
\textbf{Time scope:} Single day \\
\textbf{Need prediction:} No \\
\textbf{Need personalization:} No \\
\textbf{Need external knowledge:} No \\
\textbf{Response risk level:} Low \\[2pt]
\textbf{Execution steps:}
\begin{Enumerate}
\vspace{-0.8em}
    \item Identify the hour with maximum heart rate.
    \item Retrieve the total steps during that hour.
    \item Return the identified hour and the corresponding step count, or explicitly state if required data are missing.
\end{Enumerate}
\end{observationbox}

==> tables/tool_summary.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{p{3.0cm}p{4.2cm}}
\toprule
Capability & Example Functions \\
\midrule
Stats Calculator & sleep summaries, HR statistics \\
Temporal Profiler & trend analysis, correlations \\
Stress SVM (ML) & HRV-based stress prediction \\
Stress Tracker (ML) & history-aware stress prediction \\
Resp Screener (FM) & COVID-19 screening from audio \\
BP Predictor (FM) & PPG blood pressure estimation \\
\bottomrule
\end{tabular}
\caption{Example wearable-health skills in WEQA, spanning analytical reasoning and predictive inference across sensing modalities, including specialized machine learning (ML) and foundation models (FM). }
\label{tab:capability_summary}
\end{table}

